High Performance Algorithms for Counting Collisions and Pairwise Interactions

The problem of counting collisions or interactions is common in areas as computer graphics and scientific simulations. Since it is a major bottleneck in applications of these areas, a lot of research has been carried out on such subject, mainly focused on techniques that allow calculations to be performed within pruned sets of objects. This paper focuses on how interaction calculation (such as collisions) within these sets can be done more efficiently than existing approaches. Two algorithms are proposed: a sequential algorithm that has linear complexity at the cost of high memory usage; and a parallel algorithm, mathematically proved to be correct, that manages to use GPU resources more efficiently than existing approaches. The proposed and existing algorithms were implemented, and experiments show a speedup of 21.7 for the sequential algorithm (on small problem size), and 1.12 for the parallel proposal (large problem size). By improving interaction calculation, this work contributes to research areas that promote interconnection in the modern world, such as computer graphics and robotics.

==> algorithm/2-meminit.tex <==
%\setlength{\textfloatsep}{0pt}
%See: https://tex.stackexchange.com/questions/26521/how-to-change-the-spacing-between-figures-tables-and-text

%\RestyleAlgo{plain}
\begin{algorithm}[H]%[htb]
    \caption{Memory initialization for counting contacts.}
    \label{algorithm:memory-init}

    \footnotesize

    \SetStartEndCondition{ (}{)}{)} % Open and close conditions with ()
    \SetAlgoBlockMarkers{}{\}}      % Close blocks with }, but don't open with {, which are set up on the \SetKw
    \AlgoDisplayBlockMarkers        % Display the { }
    \SetKwFor{For}{for}{\{}{}       % Define a for block
    \SetKwIF{If}{ElseIf}{Else}{if}{\{}{else if}{else\{}{}   % Define an if...else if...else block
    \SetKwFor{While}{while}{\{}{}   % Define a while block
    \SetArgSty{textnormal}          % Remove italic font from conditions
    \SetFuncArgSty{textnormal}      % Remove italic font from function arguments
    \SetFuncSty{textit}             % Set function names as italic
    \Indm\Indm                      % Remove indentation of line numbers

    \SetKw{In}{in}

    \For{b \In beads}{
        space[b.x][b.y][b.z] = 0\;
    }
\end{algorithm}
%\RestyleAlgo{algoruled}

==> algorithm/6-proposedalgorithm2.tex <==
\begin{algorithm}[H]
    \caption[caption]{Proposed algorithm for calculating Symmetric Pairwise Interactions (SPI) for even $N$.}
    \label{algorithm:proposedcode2}

    \footnotesize

    \SetStartEndCondition{ (}{)}{)} % Open and close conditions with ()
    \SetKwFor{For}{for}{\{}{\}}     % Define a for block
    \SetKwFor{ForTwo}{for}{}{}      % Define another for block
    \SetKwIF{If}{ElseIf}{Else}{if}{}{else if}{else}{}   % Define an if...else if...else block
    \SetKwFor{While}{while}{}{}     % Define a while block
    \SetArgSty{textnormal}          % Remove italic font from conditions
    \SetFuncArgSty{textnormal}      % Remove italic font from function arguments
    \SetFuncSty{textit}             % Set function names as italic

    \SetKwFunction{int}{interact}
    \SetKw{In}{in}
    \SetKw{To}{to}
    \SetKw{Int}{int}
    \SetKw{Even}{is even}

    \For{i = 0 \To N-1}{
        \ForTwo{j = 1 \To (N-2)/2}{
            interactions += \int{obj[i], obj[(i+j)\%N]}\;
        }
        \If(\tcc*[f]{only half beads perform one more iteration}){i $<$ N/2}{
            interactions += \int{obj[i], obj[(i+N/2)\%N]}\;
        }
    }
\end{algorithm}
